Critical Hyper-Parameters: No Random, No Cry

The selection of hyper-parameters is critical in Deep Learning. Because of the long training time of complex models and the availability of compute resources in the cloud, "one-shot" optimization schemes - where the sets of hyper-parameters are selected in advance (e.g. on a grid or in a random manner) and the training is executed in parallel - are commonly used. It is known that grid search is sub-optimal, especially when only a few critical parameters matter, and suggest to use random search instead. Yet, random search can be "unlucky" and produce sets of values that leave some part of the domain unexplored. Quasi-random methods, such as Low Discrepancy Sequences (LDS) avoid these issues. We show that such methods have theoretical properties that make them appealing for performing hyperparameter search, and demonstrate that, when applied to the selection of hyperparameters of complex Deep Learning models (such as state-of-the-art LSTM language models and image classification models), they yield suitable hyperparameters values with much fewer runs than random search. We propose a particularly simple LDS method which can be used as a drop-in replacement for grid or random search in any Deep Learning pipeline, both as a fully one-shot hyperparameter search or as an initializer in iterative batch optimization.

==> detailedtoyxp.tex <==
\section{Artificial objective functions: detailed results}\label{detailedtoyxps}
This section presents detailed results of LDS, random search and other sampling methods for one-shot optimization.

\subsection{Artificial xps on quasirandom, with most important variables first for illcond}                                                             % NOTINICML
We here consider the sphere objective function (for which all variables are equally important) and the illcond objective function (for which the first variables are the most important).                                                             % NOTINICML
Results are presented in Table \ref{illcondcool}. For the sphere the best results are always obtained by a scrambled method; for illcond (for which only the few first variables matter) the best results                                                             % NOTINICML
are always obtained by a LDS and the different LDS perform equally.                                                             % NOTINICML
                                                             % NOTINICML
\begin{table*}\center                                                             % NOTINICML
{\scriptsize{                                                             % NOTINICML
\begin{tabular}{|c|c|}                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 2, sphere}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
S-SH & 0.0054$\pm$0.0001\\                                                             % NOTINICML
Hammersley & 0.0057$\pm$0.0001\\                                                             % NOTINICML
Halton & 0.0061$\pm$0.0001\\                                                             % NOTINICML
scr-Halton & 0.0062$\pm$0.0001\\                                                             % NOTINICML
scr-Halton3dmirror & 0.0063$\pm$0.0001\\                                                             % NOTINICML
sobol & 0.0074$\pm$0.0001\\                                                             % NOTINICML
Hammersley3dmirror & 0.0077$\pm$0.0001\\                                                             % NOTINICML
naivedoe3dmirror & 0.0077$\pm$0.0001\\                                                             % NOTINICML
naivedoe & 0.0080$\pm$0.0001\\                                                             % NOTINICML
S-SH3dmirror & 0.0080$\pm$0.0002\\                                                             % NOTINICML
random3dmirror & 0.0082$\pm$0.0002\\                                                             % NOTINICML
Halton3dmirror & 0.0086$\pm$0.0002\\                                                             % NOTINICML
lhs & 0.0087$\pm$0.0002\\                                                             % NOTINICML
sobol3dmirror & 0.0090$\pm$0.0002\\                                                             % NOTINICML
random & 0.0092$\pm$0.0002\\                                                             % NOTINICML
lhs3dmirror & 0.0101$\pm$0.0003\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 2, illcond}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
Hammersley & 0.0155$\pm$0.0003\\                                                             % NOTINICML
S-SH & 0.0155$\pm$0.0003\\                                                             % NOTINICML
scr-Halton & 0.0170$\pm$0.0004\\                                                             % NOTINICML
Halton & 0.0172$\pm$0.0004\\                                                             % NOTINICML
scr-Halton3dmirror & 0.0207$\pm$0.0005\\                                                             % NOTINICML
lhs3dmirror & 0.0229$\pm$0.0007\\                                                             % NOTINICML
lhs & 0.0243$\pm$0.0007\\                                                             % NOTINICML
Hammersley3dmirror & 0.0244$\pm$0.0007\\                                                             % NOTINICML
Halton3dmirror & 0.0247$\pm$0.0005\\                                                             % NOTINICML
sobol & 0.0257$\pm$0.0007\\                                                             % NOTINICML
S-SH3dmirror & 0.0259$\pm$0.0008\\                                                             % NOTINICML
sobol3dmirror & 0.0261$\pm$0.0007\\                                                             % NOTINICML
random & 0.0261$\pm$0.0008\\                                                             % NOTINICML
naivedoe3dmirror & 0.0263$\pm$0.0008\\                                                             % NOTINICML
naivedoe & 0.0275$\pm$0.0007\\                                                             % NOTINICML
random3dmirror & 0.0345$\pm$0.0011\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 4, sphere}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
S-SH & 0.0716$\pm$0.0011\\                                                             % NOTINICML
Hammersley & 0.0728$\pm$0.0011\\                                                             % NOTINICML
Halton & 0.0755$\pm$0.0013\\                                                             % NOTINICML
S-SH3dmirror & 0.0769$\pm$0.0013\\                                                             % NOTINICML
naivedoe & 0.0773$\pm$0.0013\\                                                             % NOTINICML
scr-Halton & 0.0779$\pm$0.0013\\                                                             % NOTINICML
sobol & 0.0783$\pm$0.0013\\                                                             % NOTINICML
lhs & 0.0815$\pm$0.0013\\                                                             % NOTINICML
Hammersley3dmirror & 0.0842$\pm$0.0015\\                                                             % NOTINICML
random & 0.0873$\pm$0.0017\\                                                             % NOTINICML
lhs3dmirror & 0.0906$\pm$0.0014\\                                                             % NOTINICML
naivedoe3dmirror & 0.0942$\pm$0.0018\\                                                             % NOTINICML
sobol3dmirror & 0.0974$\pm$0.0016\\                                                             % NOTINICML
Halton3dmirror & 0.1019$\pm$0.0019\\                                                             % NOTINICML
scr-Halton3dmirror & 0.1034$\pm$0.0021\\                                                             % NOTINICML
random3dmirror & 0.1311$\pm$0.0020\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 4, illcond}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
S-SH & 0.8254$\pm$0.0125\\                                                             % NOTINICML
Hammersley & 0.8475$\pm$0.0127\\                                                             % NOTINICML
sobol & 0.8791$\pm$0.0142\\                                                             % NOTINICML
scr-Halton & 0.9021$\pm$0.0157\\                                                             % NOTINICML
Halton & 0.9154$\pm$0.0161\\                                                             % NOTINICML
S-SH3dmirror & 0.9690$\pm$0.0150\\                                                             % NOTINICML
Hammersley3dmirror & 0.9949$\pm$0.0158\\                                                             % NOTINICML
naivedoe & 1.0159$\pm$0.0197\\                                                             % NOTINICML
random3dmirror & 1.0467$\pm$0.0225\\                                                             % NOTINICML
Halton3dmirror & 1.0720$\pm$0.0225\\                                                             % NOTINICML
lhs & 1.0903$\pm$0.0206\\                                                             % NOTINICML
scr-Halton3dmirror & 1.0921$\pm$0.0240\\                                                             % NOTINICML
sobol3dmirror & 1.0954$\pm$0.0229\\                                                             % NOTINICML
random & 1.1211$\pm$0.0210\\                                                             % NOTINICML
lhs3dmirror & 1.1531$\pm$0.0217\\                                                             % NOTINICML
naivedoe3dmirror & 1.8661$\pm$0.0415\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
  \end{tabular}                                                             % NOTINICML
\begin{tabular}{|c|c|}                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 8, sphere}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
scr-Halton & 0.3744$\pm$0.0040\\                                                             % NOTINICML
Halton & 0.3785$\pm$0.0039\\                                                             % NOTINICML
Hammersley & 0.3816$\pm$0.0039\\                                                             % NOTINICML
sobol & 0.3853$\pm$0.0042\\                                                             % NOTINICML
S-SH & 0.3867$\pm$0.0039\\                                                             % NOTINICML
lhs & 0.3885$\pm$0.0042\\                                                             % NOTINICML
naivedoe & 0.3995$\pm$0.0045\\                                                             % NOTINICML
random & 0.4039$\pm$0.0043\\                                                             % NOTINICML
scr-Halton3dmirror & 0.4577$\pm$0.0056\\                                                             % NOTINICML
naivedoe3dmirror & 0.4723$\pm$0.0053\\                                                             % NOTINICML
lhs3dmirror & 0.4764$\pm$0.0055\\                                                             % NOTINICML
S-SH3dmirror & 0.4780$\pm$0.0060\\                                                             % NOTINICML
sobol3dmirror & 0.4859$\pm$0.0055\\                                                             % NOTINICML
random3dmirror & 0.5038$\pm$0.0055\\                                                             % NOTINICML
Hammersley3dmirror & 0.5434$\pm$0.0068\\                                                             % NOTINICML
Halton3dmirror & 0.6133$\pm$0.0076\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 8, illcond}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
S-SH & 31.4944$\pm$0.3865\\                                                             % NOTINICML
sobol & 32.1118$\pm$0.3980\\                                                             % NOTINICML
Hammersley & 32.2906$\pm$0.3838\\                                                             % NOTINICML
Halton & 32.6409$\pm$0.3992\\                                                             % NOTINICML
scr-Halton & 32.7235$\pm$0.4049\\                                                             % NOTINICML
random & 33.5384$\pm$0.4245\\                                                             % NOTINICML
S-SH3dmirror & 33.9388$\pm$0.4340\\                                                             % NOTINICML
lhs & 34.6569$\pm$0.4283\\                                                             % NOTINICML
Hammersley3dmirror & 34.9856$\pm$0.4536\\                                                             % NOTINICML
naivedoe & 35.3151$\pm$0.4595\\                                                             % NOTINICML
scr-Halton3dmirror & 36.5532$\pm$0.4958\\                                                             % NOTINICML
Halton3dmirror & 37.8466$\pm$0.5019\\                                                             % NOTINICML
sobol3dmirror & 38.7017$\pm$0.5379\\                                                             % NOTINICML
random3dmirror & 39.1370$\pm$0.5331\\                                                             % NOTINICML
naivedoe3dmirror & 39.5667$\pm$0.5523\\                                                             % NOTINICML
lhs3dmirror & 41.4147$\pm$0.5170\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 16, sphere}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
scr-Halton & 1.2184$\pm$0.0082\\                                                             % NOTINICML
Halton & 1.2191$\pm$0.0085\\                                                             % NOTINICML
Hammersley & 1.2246$\pm$0.0085\\                                                             % NOTINICML
sobol & 1.2278$\pm$0.0081\\                                                             % NOTINICML
lhs & 1.2415$\pm$0.0080\\                                                             % NOTINICML
S-SH & 1.2427$\pm$0.0082\\                                                             % NOTINICML
random & 1.2622$\pm$0.0085\\                                                             % NOTINICML
naivedoe & 1.2679$\pm$0.0087\\                                                             % NOTINICML
S-SH3dmirror & 1.3816$\pm$0.0102\\                                                             % NOTINICML
naivedoe3dmirror & 1.3956$\pm$0.0105\\                                                             % NOTINICML
scr-Halton3dmirror & 1.4006$\pm$0.0101\\                                                             % NOTINICML
lhs3dmirror & 1.4316$\pm$0.0099\\                                                             % NOTINICML
random3dmirror & 1.4637$\pm$0.0112\\                                                             % NOTINICML
sobol3dmirror & 1.4808$\pm$0.0104\\                                                             % NOTINICML
Hammersley3dmirror & 1.6063$\pm$0.0117\\                                                             % NOTINICML
Halton3dmirror & 1.7789$\pm$0.0132\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 16, illcond}\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
Halton & 902.1823$\pm$8.2047\\                                                             % NOTINICML
scr-Halton & 902.4184$\pm$7.7450\\                                                             % NOTINICML
Hammersley & 906.3696$\pm$7.9888\\                                                             % NOTINICML
sobol & 906.6517$\pm$7.9694\\                                                             % NOTINICML
S-SH & 911.5179$\pm$7.8684\\                                                             % NOTINICML
naivedoe & 923.0551$\pm$8.6561\\                                                             % NOTINICML
lhs & 943.5814$\pm$8.7329\\                                                             % NOTINICML
scr-Halton3dmirror & 959.4747$\pm$9.9572\\                                                             % NOTINICML
random & 961.8339$\pm$9.4571\\                                                             % NOTINICML
S-SH3dmirror & 966.8579$\pm$9.6211\\                                                             % NOTINICML
lhs3dmirror & 1001.8826$\pm$9.2670\\                                                             % NOTINICML
sobol3dmirror & 1036.8494$\pm$10.1964\\                                                             % NOTINICML
naivedoe3dmirror & 1072.3794$\pm$11.1683\\                                                             % NOTINICML
Hammersley3dmirror & 1108.8699$\pm$10.7105\\                                                             % NOTINICML
random3dmirror & 1169.4045$\pm$12.2632\\                                                             % NOTINICML
Halton3dmirror & 1196.2969$\pm$11.4930\\                                                             % NOTINICML
	\hline                                                             % NOTINICML
	\end{tabular}                                                             % NOTINICML
  }}                                                             % NOTINICML
  \caption{\label{illcondcool}Minimum sampled objective function for the sphere function and for the illcond function (illcond has the most important variables first), but budget 37.}                                                             % NOTINICML
\end{table*}                                                             % NOTINICML
                                                             % NOTINICML
\subsection{Artificial xps on quasirandom, with most important variables last for illcond (reverseIllcond)}                                                             % NOTINICML
We recommended to use most critical variables first (section \ref{ordering});                                                              % NOTINICML
we here check results when the objective function is designed in a complete opposite manner, i.e.                                                              % NOTINICML
most important variables last - this is the case in which the user did not manage to properly rank the importance of variables.                                                              % NOTINICML
                                                             % NOTINICML
Consistently with theory, results (Table \ref{illcondnotcool}) for Halton and Hammersley are way worse than random at least in high dimension - whereas for illcond (previous section) Halton \& Hammersley were consistently better than random. On the other hand, scrambled variants and Sobol perform quite well - also consistently with theory as scrambling is aimed at improving results in high dimension.                                                             % NOTINICML
\begin{table*}\center                                                             % NOTINICML
{\scriptsize{                                                             % NOTINICML
\begin{tabular}{|c|c|}                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 2}\\                                                             % NOTINICML
\hline                                                             % NOTINICML
S-SH & 0.0160$\pm$0.0003\\                                                             % NOTINICML
Hammersley & 0.0166$\pm$0.0004\\                                                             % NOTINICML
Halton & 0.0172$\pm$0.0004\\                                                             % NOTINICML
scr-Halton & 0.0175$\pm$0.0004\\                                                             % NOTINICML
scr-Halton3dmirror & 0.0186$\pm$0.0004\\                                                             % NOTINICML
naivedoe & 0.0219$\pm$0.0005\\                                                             % NOTINICML
sobol & 0.0220$\pm$0.0005\\                                                             % NOTINICML
naivedoe3dmirror & 0.0236$\pm$0.0006\\                                                             % NOTINICML
Hammersley3dmirror & 0.0240$\pm$0.0006\\                                                             % NOTINICML
random & 0.0241$\pm$0.0006\\                                                             % NOTINICML
lhs & 0.0247$\pm$0.0007\\                                                             % NOTINICML
S-SH3dmirror & 0.0250$\pm$0.0006\\                                                             % NOTINICML
random3dmirror & 0.0275$\pm$0.0007\\                                                             % NOTINICML
lhs3dmirror & 0.0278$\pm$0.0008\\                                                             % NOTINICML
Halton3dmirror & 0.0286$\pm$0.0007\\                                                             % NOTINICML
sobol3dmirror & 0.0306$\pm$0.0008\\                                                             % NOTINICML
\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 4}\\                                                             % NOTINICML
\hline                                                             % NOTINICML
Hammersley & 0.8421$\pm$0.0139\\                                                             % NOTINICML
S-SH & 0.8950$\pm$0.0148\\                                                             % NOTINICML
Halton & 0.9280$\pm$0.0168\\                                                             % NOTINICML
scr-Halton & 0.9343$\pm$0.0160\\                                                             % NOTINICML
sobol & 0.9534$\pm$0.0172\\                                                             % NOTINICML
lhs & 1.0184$\pm$0.0191\\                                                             % NOTINICML
naivedoe & 1.0913$\pm$0.0206\\                                                             % NOTINICML
S-SH3dmirror & 1.3770$\pm$0.0277\\                                                             % NOTINICML
sobol3dmirror & 1.4108$\pm$0.0275\\                                                             % NOTINICML
scr-Halton3dmirror & 1.5129$\pm$0.0376\\                                                             % NOTINICML
Hammersley3dmirror & 1.5228$\pm$0.0342\\                                                             % NOTINICML
random & 1.5522$\pm$0.0504\\                                                             % NOTINICML
lhs3dmirror & 1.6735$\pm$0.0336\\                                                             % NOTINICML
naivedoe3dmirror & 1.7350$\pm$0.0334\\                                                             % NOTINICML
Halton3dmirror & 1.9037$\pm$0.0581\\                                                             % NOTINICML
random3dmirror & 2.1842$\pm$0.0707\\                                                             % NOTINICML
\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
\begin{tabular}{|c|c|}                                                             % NOTINICML
	\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 8}\\                                                             % NOTINICML
\hline                                                             % NOTINICML
sobol & 32.6119$\pm$0.3941\\                                                             % NOTINICML
naivedoe & 33.9010$\pm$0.4585\\                                                             % NOTINICML
lhs & 35.8900$\pm$0.4947\\                                                             % NOTINICML
S-SH & 36.0995$\pm$0.4765\\                                                             % NOTINICML
scr-Halton & 36.1118$\pm$0.4796\\                                                             % NOTINICML
random & 37.3243$\pm$0.5617\\                                                             % NOTINICML
Hammersley & 38.2483$\pm$0.5640\\                                                             % NOTINICML
Halton & 47.0927$\pm$0.7619\\                                                             % NOTINICML
lhs3dmirror & 59.1168$\pm$0.8528\\                                                             % NOTINICML
random3dmirror & 59.5059$\pm$0.8462\\                                                             % NOTINICML
scr-Halton3dmirror & 62.5933$\pm$0.9385\\                                                             % NOTINICML
S-SH3dmirror & 63.3482$\pm$1.0009\\                                                             % NOTINICML
sobol3dmirror & 64.7354$\pm$0.9509\\                                                             % NOTINICML
naivedoe3dmirror & 65.5584$\pm$0.8925\\                                                             % NOTINICML
Hammersley3dmirror & 78.7774$\pm$1.2885\\                                                             % NOTINICML
Halton3dmirror & 99.5334$\pm$1.7559\\                                                             % NOTINICML
\hline                                                             % NOTINICML
\multicolumn{2}{c}{Ranking in dimension 16}\\                                                             % NOTINICML
\hline                                                             % NOTINICML
S-SH & 902.1689$\pm$8.1918\\                                                             % NOTINICML
sobol & 926.6286$\pm$8.0765\\                                                             % NOTINICML
naivedoe & 938.6190$\pm$8.2898\\                                                             % NOTINICML
scr-Halton & 939.7127$\pm$8.8606\\                                                             % NOTINICML
lhs & 947.1720$\pm$9.0711\\                                                             % NOTINICML
random & 970.2377$\pm$9.5650\\                                                             % NOTINICML
scr-Halton3dmirror & 1323.8852$\pm$13.4973\\                                                             % NOTINICML
lhs3dmirror & 1350.1251$\pm$12.4491\\                                                             % NOTINICML
Hammersley & 1366.7788$\pm$15.4354\\                                                             % NOTINICML
sobol3dmirror & 1368.4549$\pm$12.4128\\                                                             % NOTINICML
S-SH3dmirror & 1369.0838$\pm$13.7944\\                                                             % NOTINICML
random3dmirror & 1369.8667$\pm$13.6301\\                                                             % NOTINICML
Halton & 1397.1004$\pm$15.9877\\                                                             % NOTINICML
naivedoe3dmirror & 1411.1522$\pm$14.8934\\                                                             % NOTINICML
Halton3dmirror & 1818.1474$\pm$19.1002\\                                                             % NOTINICML
Hammersley3dmirror & 1831.8963$\pm$20.3880\\                                                             % NOTINICML
\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
}}                                                             % NOTINICML
\caption{\label{illcondnotcool}Best sampled point for the reverse illcond function, i.e. when most important variables are last - results are much worse, for quasirandom, that when they were ranked first. Smaller values for better results. Scrambled variants of Halton/Hammersley and Sobol resist much better than Halton/Hammersley. Mirrored samplers fail.}                                                             % NOTINICML
\end{table*}                                                             % NOTINICML
                                                             % NOTINICML
                                                             % NOTINICML
\subsection{Antisobol: a deceptive function for Sobol for one shot optimization}                                                             % NOTINICML
Table \ref{antisobol} presents results on the antisobol function, build as a deceptive function for the Sobol implementation we use - noticeably, results might depend on the direction vectors.                                                             % NOTINICML
HY refers to Hammersley, ND to Naive-Doe, S to Sobol, HN to Halton, SHN to Scrambled-Halton. The "S-" for random shift is discarded in this section and in the next section as all LDS in the present xps are randomly shifted. We see clearly disappointing results for Sobol, and excellent results for S-SH.                                                             % NOTINICML
%\setlength{\tabcolsep}{0.1em}                                                             % NOTINICML
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}                                                             % NOTINICML
                                                             % NOTINICML
\begin{table*}                                                             % NOTINICML
	\center                                                             % NOTINICML
	\small                                                             % NOTINICML
	\begin{tabular}{ccccccccccccccccHHHHHHHHHHHHHHH}                                                             % NOTINICML
\hline                                                             % NOTINICML
	Dim & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
	2 & {\bf\em{R}} & HY & HY & SH & SH & SH & ND & SH & SH & HY & SH & HY & {\bf\em{R}} & SH & SH & SH & lhs & HY & SH & SH & HY & HY & HY & HY & HY & HY & SH & HY & SH & HY \\                                                             % NOTINICML
	3 & SH & SH & SH & HY & SH & SH & ND & ND & HY & SH & HY & SH & SH & ND & SH & lhs & SH & HY & SH & HY & ND & HY & SH & SH & lhs & SH & SH & SH & ND & SH \\                                                             % NOTINICML
	4 & SH & HY & lhs & HY & SH & HY & HY & {\bf\em{R}} & HY & HY & HY & SH & SH & HY & HY & SH & SH & HY & SH & HY & HY & lhs & HY & HY & HY & HY & SH & SH & lhs & SH \\                                                             % NOTINICML
	5 & SH & HY & lhs & HY & SH & HY & SH & ND & lhs & SH & HY & lhs & HY & HY & SH & HY & HY & SH & SH & HY & HY & HY & SH & SH & SH & SH & SH & HY & SH & HY \\                                                             % NOTINICML
	6 & SH & HY & {\bf\em{R}} & HY & SH & SH & HY & HY & SH & SH & HY & SH & SH & SH & SH & SH & HY & SH & {\bf\em{R}} & HY & lhs & SH & SH & HY & HY & HY & SH & HY & HY & HY \\                                                             % NOTINICML
	7 & SH & HY & HY & SH & SH & HY & SH & HY & {\bf\em{R}} & HY & SH & SH & HY & HY & HY & SH & HY & SH & SH & SH & HY & HY & HY & SH & HY & {\bf\em{R}} & HY & HY & HY & SH \\                                                             % NOTINICML
	8 & HY & HY & HY & HY & HY & ND & SH & SH & {\bf\em{R}} & SH & HY & SH & HY & HY & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & SH & SH & HY & HY & HY & HY & HY & SH & {\bf\em{R}} & HY & HY & HY & HY \\                                                             % NOTINICML
	9 & SH & HY & SH & SH & SH & HY & SH & SH & lhs & HY & SH & SH & HY & SH & lhs & SH & HY & HY & SH & SH & {\bf\em{R}} & HY & SH & SH & HY & HY & SH & {\bf\em{R}} & SH & HY \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
                                                             % NOTINICML
	\begin{tabular}{cHHHHHHHHHHHHHHHccccccccccccccc}                                                             % NOTINICML
\hline                                                             % NOTINICML
	Dim & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
	2 & {\bf\em{R}} & HY & HY & SH & SH & SH & ND & SH & SH & HY & SH & HY & {\bf\em{R}} & SH & SH & SH & lhs & HY & SH & SH & HY & HY & HY & HY & HY & HY & SH & HY & SH & HY \\                                                             % NOTINICML
	3 & SH & SH & SH & HY & SH & SH & ND & ND & HY & SH & HY & SH & SH & ND & SH & lhs & SH & HY & SH & HY & ND & HY & SH & SH & lhs & SH & SH & SH & ND & SH \\                                                             % NOTINICML
	4 & SH & HY & lhs & HY & SH & HY & HY & {\bf\em{R}} & HY & HY & HY & SH & SH & HY & HY & SH & SH & HY & SH & HY & HY & lhs & HY & HY & HY & HY & SH & SH & lhs & SH \\                                                             % NOTINICML
	5 & SH & HY & lhs & HY & SH & HY & SH & ND & lhs & SH & HY & lhs & HY & HY & SH & HY & HY & SH & SH & HY & HY & HY & SH & SH & SH & SH & SH & HY & SH & HY \\                                                             % NOTINICML
	6 & SH & HY & {\bf\em{R}} & HY & SH & SH & HY & HY & SH & SH & HY & SH & SH & SH & SH & SH & HY & SH & {\bf\em{R}} & HY & lhs & SH & SH & HY & HY & HY & SH & HY & HY & HY \\                                                             % NOTINICML
	7 & SH & HY & HY & SH & SH & HY & SH & HY & {\bf\em{R}} & HY & SH & SH & HY & HY & HY & SH & HY & SH & SH & SH & HY & HY & HY & SH & HY & {\bf\em{R}} & HY & HY & HY & SH \\                                                             % NOTINICML
	8 & HY & HY & HY & HY & HY & ND & SH & SH & {\bf\em{R}} & SH & HY & SH & HY & HY & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & SH & SH & HY & HY & HY & HY & HY & SH & {\bf\em{R}} & HY & HY & HY & HY \\                                                             % NOTINICML
	9 & SH & HY & SH & SH & SH & HY & SH & SH & lhs & HY & SH & SH & HY & SH & lhs & SH & HY & HY & SH & SH & {\bf\em{R}} & HY & SH & SH & HY & HY & SH & {\bf\em{R}} & SH & HY \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
                                                             % NOTINICML
                                                             % NOTINICML
                                                             % NOTINICML
	\caption{\label{antisobol}Best performing method, for each of 30 runs (one column per run), among the 8 presented methods, on the Antisobol function. Sobol performs poorly (never visible in the table), whereas random (R) is present several times. Randomly shifted scrambled Hammersley (denoted SH for short in the table) performs very well.}                                                             % NOTINICML
\end{table*}                                                             % NOTINICML
                                                             % NOTINICML
                                                             % NOTINICML
\subsection{Antish: Deceptive function for randomly shifted Scrambled-Hammersley}                                                             % NOTINICML
                                                             % NOTINICML
In Table \ref{antish}, dedicated to results on the Antish function made for being deceptive for S-SH, R wins 39 times, whereas SH wins 11 times and SHN wins 14 times; these scrambled variants of HN together win only 25 times - this shows that the Antish function is deceptive for S-SH and S-Halton.                                                              % NOTINICML
\begin{table*}\center                                                             % NOTINICML
	\scriptsize                                                             % NOTINICML
\begin{tabular}{ccccccccccccccccHHHHHHHHHHHHHHH}                                                             % NOTINICML
\hline                                                             % NOTINICML
	Dim & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
	12 & lhs & {\bf\em{R}} & {\bf\em{R}} & ND & lhs & ND & ND & S & ND & ND & ND & {\bf\em{R}} & {\bf\em{SH}} & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & S & lhs & S & lhs & lhs & {\bf\em{SHN}} & S & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & S & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	13 & {\bf\em{SHN}} & S & lhs & {\bf\em{R}} & S & lhs & lhs & lhs & lhs & lhs & lhs & lhs & {\bf\em{R}} & S & ND & lhs & lhs & lhs & S & S & lhs & ND & {\bf\em{SH}} & S & {\bf\em{R}} & lhs & S & lhs & {\bf\em{SH}} & S \\                                                             % NOTINICML
	14 & lhs & {\bf\em{R}} & S & S & lhs & S & {\bf\em{R}} & S & ND & lhs & S & lhs & {\bf\em{SH}} & {\bf\em{R}} & S & ND & S & ND & ND & {\bf\em{R}} & lhs & S & {\bf\em{R}} & {\bf\em{R}} & ND & {\bf\em{SHN}} & lhs & lhs & S & S \\                                                             % NOTINICML
	15 & S & lhs & ND & ND & lhs & ND & lhs & lhs & lhs & lhs & S & lhs & ND & S & ND & S & S & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{SH}} & lhs & {\bf\em{R}} & {\bf\em{R}} & S & S & S & {\bf\em{SHN}} & {\bf\em{R}} & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	16 & ND & {\bf\em{SH}} & {\bf\em{SHN}} & S & ND & {\bf\em{R}} & ND & ND & ND & lhs & lhs & ND & {\bf\em{R}} & ND & ND & ND & S & ND & {\bf\em{SHN}} & {\bf\em{SH}} & {\bf\em{R}} & S & S & {\bf\em{R}} & ND & S & {\bf\em{SHN}} & lhs & lhs & lhs \\                                                             % NOTINICML
	17 & lhs & S & lhs & S & ND & {\bf\em{R}} & lhs & S & S & S & ND & lhs & {\bf\em{SHN}} & lhs & lhs & {\bf\em{SH}} & {\bf\em{SHN}} & S & S & {\bf\em{R}} & S & ND & lhs & {\bf\em{SHN}} & {\bf\em{R}} & {\bf\em{R}} & lhs & S & ND & {\bf\em{R}} \\                                                             % NOTINICML
	18 & {\bf\em{R}} & ND & ND & S & S & {\bf\em{R}} & {\bf\em{R}} & ND & {\bf\em{R}} & ND & lhs & ND & {\bf\em{SHN}} & ND & S & S & S & lhs & {\bf\em{SHN}} & {\bf\em{R}} & S & {\bf\em{R}} & {\bf\em{SHN}} & {\bf\em{SHN}} & lhs & ND & lhs & lhs & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
\begin{tabular}{cHHHHHHHHHHHHHHHccccccccccccccc}                                                             % NOTINICML
\hline                                                             % NOTINICML
	Dim & & & & & & & & & & & & & & & & & & & & & & & & & & & & & \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
	12 & lhs & {\bf\em{R}} & {\bf\em{R}} & ND & lhs & ND & ND & S & ND & ND & ND & {\bf\em{R}} & {\bf\em{SH}} & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & S & lhs & S & lhs & lhs & {\bf\em{SHN}} & S & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{R}} & S & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	13 & {\bf\em{SHN}} & S & lhs & {\bf\em{R}} & S & lhs & lhs & lhs & lhs & lhs & lhs & lhs & {\bf\em{R}} & S & ND & lhs & lhs & lhs & S & S & lhs & ND & {\bf\em{SH}} & S & {\bf\em{R}} & lhs & S & lhs & {\bf\em{SH}} & S \\                                                             % NOTINICML
	14 & lhs & {\bf\em{R}} & S & S & lhs & S & {\bf\em{R}} & S & ND & lhs & S & lhs & {\bf\em{SH}} & {\bf\em{R}} & S & ND & S & ND & ND & {\bf\em{R}} & lhs & S & {\bf\em{R}} & {\bf\em{R}} & ND & {\bf\em{SHN}} & lhs & lhs & S & S \\                                                             % NOTINICML
	15 & S & lhs & ND & ND & lhs & ND & lhs & lhs & lhs & lhs & S & lhs & ND & S & ND & S & S & {\bf\em{R}} & {\bf\em{R}} & {\bf\em{SH}} & lhs & {\bf\em{R}} & {\bf\em{R}} & S & S & S & {\bf\em{SHN}} & {\bf\em{R}} & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	16 & ND & {\bf\em{SH}} & {\bf\em{SHN}} & S & ND & {\bf\em{R}} & ND & ND & ND & lhs & lhs & ND & {\bf\em{R}} & ND & ND & ND & S & ND & {\bf\em{SHN}} & {\bf\em{SH}} & {\bf\em{R}} & S & S & {\bf\em{R}} & ND & S & {\bf\em{SHN}} & lhs & lhs & lhs \\                                                             % NOTINICML
	17 & lhs & S & lhs & S & ND & {\bf\em{R}} & lhs & S & S & S & ND & lhs & {\bf\em{SHN}} & lhs & lhs & {\bf\em{SH}} & {\bf\em{SHN}} & S & S & {\bf\em{R}} & S & ND & lhs & {\bf\em{SHN}} & {\bf\em{R}} & {\bf\em{R}} & lhs & S & ND & {\bf\em{R}} \\                                                             % NOTINICML
	18 & {\bf\em{R}} & ND & ND & S & S & {\bf\em{R}} & {\bf\em{R}} & ND & {\bf\em{R}} & ND & lhs & ND & {\bf\em{SHN}} & ND & S & S & S & lhs & {\bf\em{SHN}} & {\bf\em{R}} & S & {\bf\em{R}} & {\bf\em{SHN}} & {\bf\em{SHN}} & lhs & ND & lhs & lhs & lhs & {\bf\em{SH}} \\                                                             % NOTINICML
	\hline                                                             % NOTINICML
\end{tabular}                                                             % NOTINICML
	\caption{\label{antish}Best method for different runs of different dimensions, on the AntiSh function designed for being deceptive for the randomly shifted Scrambled Hammersley. Each column corresponds to one of 30 runs, each row corresponds to a different dimensionality. Each cell shows which method performed best. Random performed well overall, but the gap with randomly shifted scrambled Hammersley (denoted SH in the present table) is small, whereas in Fig. \ref{antisobol} we could exhibit a function for which Sobol performed very poorly - it seems easier to find counterexamples for Sobol than for SH (at least, for the version of Sobol we use, and for SH with random scrambling and randomly shifted).}                                                             % NOTINICML
\end{table*}                                                             % NOTINICML



==> zetab.tex <==
	\begin{table}
		\scriptsize\centering
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		Setting       & Budgets              &                 & Average     &  Robustness \\
		                  &                            & Speed-up & speed-up   &  speed-up     \\
				  \hline
				  \hline
				  Untuned*         & 5:12        & +350\%    & & \\    %p-value 0.049
				  (3 HP, 7 epochs) &                &                  &            & \\
				  \hline
				  Untuned*         & 5:15, 17, 19 & +237\% & & \\    % p-value 0.03
				  (3 HP, 7 epochs) &          &               &            & \\
				  \hline
%				  Tuned  & & & & \\    
%				  (3HP, 7 epochs)*            & 5:20        & -50.0\%       & &   \\  pvalue 0.17 not signif for speedup
%				  (3 HP, 7 epochs)***         & 5:47        & -51\%    &  & +28\% \\  pvalue 0.18 not signif for speedup
				  \hline
				  Tuned***         & 48:73      & +87\%   &  & +50\% \\    % p-value < 0.05 by far
				  (3 HP, 7 epochs) &                &                  &            &   \\
				  \hline
				  Untuned*   & 25:5:145    & +12.8 \% & +19.5\%      & +26\%    \\   %%%% Fig. 7 cool   %p-value not signif for su
				  (3 HP, 7 epochs) &       &                 &                    &               \\
				  \hline
				  Half-tuned*& 40:10:120   & +50.0 \% & +19.5\%    & +25\%    \\   %%%% Fig. 8 very cool
				   (3 HP, 7 epochs)        & and 140:20:200 &                &                  &                \\
				   \hline
				   Leaky**    & 10:5:100   &  +62 \% & +40\% & +40\% \\  %%% Figure 5
				   (5 HP, 30 epochs)       &                  &               &            &            \\
           \hline
           PTB Bytes/Words & budget 20  & +57\% & +57\% & +57\% \\   %%% 22/36 
           (7 HP, 17 epochs)  & budget 30  & +0\% & +0\% & +0\% \\   %%% 
           (36 xps) & & & & \\
\hline
Tuned*           & 20:5:30     & +160\%  & +160\% & +160\%  \\
(3 HP, 4 epochs) &             &         &        &         \\
\hline
	\end{tabular}
		(only rows with p-values $<$ 0.05 are kept)
		\begin{tabular}{|c|c|c|c|c|}
			\hline
			          & PTB & PTB & UBPTB & UBPTB \\
				  & Bytes & Words & Bytes & Words \\
			\hline
			Budget 15 & S-SH & S-SH & S-SH & S-SH \\
			\hline
			Budget 60 & S-SH & S-SH & S-SH & S-SH \\
			\hline
		\end{tabular}\\
		Overall p-value: 0.004.
		\begin{tabular}{|c|c|c|}
			\hline
			7 HP	& budget 30      & budget 20 \\
			(see SM)& bytes \& words & bytes \& words \\
			\hline
			S-SH vs random & (+0\%) & +57\%  \\
			\hline
			S-SH vs Halton & (+12\%) \% & +127\%  \\
			\hline
		\end{tabular}\\
		P-values between parentheses are not signif. ($>0.05$).
		\caption{\label{main}Table of results for the speed-up of S-SH compared to random (top) and best method among S-SH and pure random in terms of average test error over 35 runs in 8 cases (middle****) and speed-ups for 36 xps with 7 HP (bottom, on PTB; we added Adam's epsilon parameter, dropout probability, learning rate decay, epoch at which the decay starts). P-values are computed by Fisher's exact test, for the null hypothesis that the frequency of speed-up $>0$ (among speed-up $\neq 0$) is $\frac12$ (top and bottom); see text and SM for detailed setup, additional xps, additional statistical validations and curves. The 36 xps correspond to different numbers of units. Top: the two last rows have the same values for different speed-ups because there is only one LDS and one instance of random search (other rows have 3 instances of random search). Many experiments have a small number of epochs, but all experiments (see text and SM) with larger number of epochs ($17$ to $45$) have speedup $\geq 0$ for LDS.}
	\end{table}

